A practical example for the non-linear Bayesian filtering of model parameters

In this tutorial we consider the non-linear Bayesian filtering of static parameters in a time-dependent model. We outline the theoretical background and discuss appropriate solvers. We focus on particle-based filters and present Sequential Importance Sampling (SIS) and Sequential Monte Carlo (SMC). Throughout the paper we illustrate the concepts and techniques with a practical example using real-world data. The task is to estimate the gravitational acceleration of the Earth $g$ by using observations collected from a simple pendulum. Importantly, the particle filters enable the adaptive updating of the estimate for $g$ as new observations become available. For tutorial purposes we provide the data set and a Python implementation of the particle filters.

==> sections/1_intro.tex <==
\section{Introduction}

An important building block of uncertainty quantification is the statistical estimation and sustained learning of parameters in mathematical and computational models.
In science and engineering models are used to emulate, predict, and optimise the behavior of a system of interest.
Examples include the transport of contaminants by groundwater flow in hydrology, the price of a European option in finance, or the motion of stars and planets by mutual gravitational forces in astrophysics. 
The associated mathematical models for these examples are an elliptic partial differential equation (PDE), the parabolic Black-Scholes PDE, and a system of ordinary differential equations (ODEs) describing the $N$-body dynamics.

%In practice, models are often used for predictions and investigations in a particular setting.
Assuming that we have observational data of the system of interest it is now necessary to calibrate the model with respect to these observations.
This means that we identify model parameters such that the model output is close to the observations in a suitable metric.
In the examples above we need to calibrate the hydraulic conductivity of the groundwater reservoir, the volatility of the stock associated with the option, and the masses of the interstellar bodies.

In this tutorial  we focus on the next step following the model calibration, namely the updating of the estimated parameters as additional observations become available.
This is an important task since many systems are only partially observed. 
Thus it is often unlikely to obtain high quality estimates of underlying model parameters by using only a single data set.
Moreover, it is often very expensive or impossible  to restart the parameter estimation with all data sets after a new data set becomes available.
The problem of combining a parameter estimate with a new set of observations to update the estimate based on all observations is called \emph{filtering} in statistics.
Filtering can be considered as a \emph{learning process}: a certain state of knowledge based on previous observations is combined with new observations to reach an improved state of knowledge.
%A model for which parameters have been calibrated already could be interpreted as an `adult model'.
%Continuing to incorporate data into the model would then be seen as adult education. 
%In order to describe this, we have chosen to borrow the term \emph{lifelong learning} from education science, where it describes adult education (among other things).

Throughout this tutorial we consider a practical example for filtering. 
We study the periodic motion of a pendulum.
The underlying mathematical model is an ODE.
The model parameters are the length of the pendulum string $\ell$, and the gravitational acceleration of the Earth $g$.
We assume that $\ell$ is known, however, we are uncertain about $g \approx 9.81 m/s^2$. 
Our goal is to estimate and update the estimate for $g$ based on real-world observational data.
Importantly, the pendulum experiment can be carried out without expensive equipment or time-consuming preparations.
Moreover, the mathematical model is simple and does not require sophisticated or expensive numerical solvers.
However, the filtering problem is non-linear and non-Gaussian.
It does not have an analytic solution, and an efficient approximate solution must be constructed. 
We use particle filters for this task. 

The simple pendulum setting allows us to focus on the statistical aspects of the estimation problem and the construction of particle filters.
The filters we discuss, SIS and SMC, are not new, however, they deserve to be known and used by applied mathematicians working in the field of uncertainty quantification.
This tutorial enables interested readers to learn the building blocks of particle filters illustrated by a simple example.
Moreover, by providing the source code the reader can combine the filters with more sophisticated mathematical models.
\todo{
Tutorials: \cite{Doucet2011}

Textbooks: \cite{Sarkka2013} focuses on state space estimation, pendulum example, chapter on parameter estimation; \cite{Law2015} state space estimation
}

The remaining part of this tutorial is organised as follows. 
In \S \ref{Subs_Problem_Form} we give a precise formulation of the filtering problem and define a filter.
We introduce the pendulum problem in \S \ref{SubSec_Pendulum}.
In addition, we briefly discuss a tumor filtering problem from biomedical engineering.
We review previous work on model calibration, filtering and the numerical approximation of these procedures.
In \S \ref{Sec_Bayes} we introduce the Bayesian solution to the filtering problem.% in \S \ref{Subs_Problem_Form}.
Furthermore, we explain the statistical modeling of the pendulum filtering problem.
%Typically, there is no analytical solution to non-linear Bayesian filtering problems.
In \S \ref{Sec_SMC} we discuss particle-based filters, namely Sequential Importance Sampling and Sequential Monte Carlo.
We then apply both these methods to the pendulum filtering, and comment on the estimation results.
Finally, in \S \ref{sec:discussion} we discuss challenges for current filtering problems in uncertainty quantification.

\section{The filtering problem}
%\subsection{Problem formulation}
\label{Subs_Problem_Form}
We motivated the filtering of model parameters in the preceding section. 
Now we give a rigorous introduction to filtering.
Note that we first define the filtering problem in a general setting. 

Let $X$ and $H$ be separable Banach spaces.
$X$ denotes the \emph{parameter space}, and $H$ denotes the \emph{model output space}.
We define a \emph{mathematical model} $G: X \rightarrow H$ as a mapping from the parameter space to the model output space. 
Next, we observe the system of interest that is represented by the model.
We collect measurements at $T \in \mathbb{N}$ points in time $t = 1,\dots,T$. 
These observations are denoted by $y_1, y_2,\dots,y_T$. 
Each observation $y_t$ is an element of a \emph{finite-dimensional} Banach space $Y_t$.
The family of spaces $Y_1,\dots,Y_T$ are the so called \emph{data spaces}.
We model the observations by \emph{observation operators} $\mathcal{O}_t: H \rightarrow Y_t$, $t \geq 1$, that map the model output to the associated observation. 
Furthermore, we define a family of \emph{forward response operators} $\mathcal{G}_t := \mathcal{O}_t \circ G$, $t \geq 1$, that map from the parameter space directly to the associated data space.
We assume that the observations are noisy and model this fact by randomness.
The randomness is represented on an underlying probability space $(\Omega, \mathcal{A}, \mathbb{P})$.
Each observation $y_t$ is the realisation of a random variable $\widetilde{y}_t: \Omega \rightarrow Y_t$.
Moreover,
\begin{equation}
\widetilde{y}_t \sim L_t(\cdot|\theta^\dagger)
\end{equation}
where $L_t: Y_t \times X \rightarrow [0, \infty)$, $t \geq 1$, is a parameterised probability density function (w.r.t. the Lebesgue measure). 
$\theta^\dagger$ denotes the true parameter associated with the (noise-free) observations.

\begin{example}[Additive Gaussian noise] \label{Example_Gaussian_noise_add}
A typical assumption is that the measurement noise is Gaussian and additive. 
In that case $y_t$ is a realisation of the random variable
$\widetilde{y}_t = \mathcal{G}_t(\theta^\dagger) + \eta_t$,
where $\eta_t \sim \mathrm{N}(0,\Gamma_t)$ and $\Gamma_t: Y_t \rightarrow Y_t$ is a linear, symmetric, positive definite covariance operator, $t \geq 1$.
It holds
$$L_t(y_t|\theta) 
= \exp\left(-\frac{1}{2}\|\Gamma^{-1/2}(\mathcal{G}_t(\theta)-y_t)\|^2 \right).$$
\end{example}

The \emph{inverse} or \emph{smoothing problem} at a specific timepoint $t \geq 1$ is the task to  identify the unknown true parameter $\theta^\dagger$ given the data set $(y_1,\dots,y_t) =: y_{1:t}$.
We denote the estimate for the parameter by $\widehat{\theta}(y_{1:t})$. 
Hence, a formal expression for smoothing is the map $$y_{1:t} \mapsto \widehat{\theta}(y_{1:t}).$$
The \emph{filtering problem}, on the other hand, is the task to update the estimate $\widehat{\theta}(y_{1:t})$ after the observation $y_{t+1}$ is available. 
Hence, a formal expression for a \emph{filter} is the map $$\{\widehat{\theta}(y_{1:t}), y_{t+1}\}  \mapsto \widehat{\theta}(y_{1:t+1}).$$
Filtering can be considered as a \emph{learning process} in the following sense.
Our point of departure is a current state of knowledge represented by the parameter estimate $\widehat{\theta}(y_{1:t})$.
This involves all observations up to the point in time $t$.
The data set $y_{t+1}$ is then used to arrive at a new state of knowledge represented by the updated parameter estimate $\widehat{\theta}(y_{1:t+1})$.
We depict this learning process in Fig. \ref{Fig_tikz_learning}. 
\begin{figure}[htb]
\centering
\begin{tikzpicture}[scale=0.6]
\draw	(1.5,0)node[anchor=east] {timeline:};

 \draw	(1.5,-1)node[anchor=east] {state of knowledge:};
 %\draw[line width = 1.5, color = black,->](0,-1) -- (1.5,-1);
 
 \draw	(4.75,-1)node[rectangle,anchor=west,text width=1.1cm, thick,draw=black,align=center,fill=white] {$\widehat{\theta}(y_{1:t})$};
 
  \draw	(3,0.35)node[align=center] {$t$};
  
   
    \draw	(15,0.35)node[align=center] {$t+2$};
  \draw[line width = 1.0, color = black,-](3,0.1) -- (3,-0.1);
    \draw[line width = 1.0, color = black,-](9,0.1) -- (9,-0.1);
    \draw[line width = 1.0, color = black,-](15,0.1) -- (15,-0.1);

 
  \draw[line width = 1.5, color = black,->](7.5,-1) -- (10.7,-1);
    \draw[line width = 1.0, color = black,->](2,0) -- (16.5,0);

  
    \draw[line width = 1.5, color = black,<-](9,-1.65) -- (9,-2.5);
      \draw	(9,-3)node[align=center] {$y_{t+1}$};
\draw	(8,-1)node[align=center,rectangle,anchor=west,thick,draw=black,fill=white] {\scriptsize Learning};
   \draw	(11.25,-1)node[align=center,rectangle,anchor=west,text width=1.2cm,thick,draw=black,fill=white] {$\widehat{\theta}(y_{1:t+1})$};
      \draw	(9,0.35)node[align=center] {$t+1$};
 \end{tikzpicture}
 \caption{The filtering problem. The starting point is the current state of knowledge $\widehat{\theta}(y_{1:t})$ at the point in time $t$. At the timepoint $t+1$ we observe $y_{t+1}$. We want to use these observations to improve our knowledge concerning $\theta^\dagger$. The new state of knowledge is given by the updated estimate $\widehat{\theta}(y_{1:t+1})$. }
\label{Fig_tikz_learning}
\end{figure}

\subsection{A practical example}\label{SubSec_Pendulum}
In this section we describe a simple yet practical filtering problem that is associated with a real-world experiment and data.
Throughout this tutorial we will come back to this problem to illustrate the filtering of model parameters.

\begin{example}[Pendulum]%\label{Subsubsec_Pendulum_introd}
The goal of the pendulum inverse problem is the estimation of the Earth’s gravitational acceleration $g^\dagger \approx 9.81m/s^2$ using measurements collected from the periodic motion of a pendulum. 
We use a simplified model to describe the dynamics of the pendulum.
Specifically, we ignore friction, and assume that the pendulum movements take place in a twodimensional, vertically oriented plane. 
In this case the state of the pendulum can be described by a single scalar that is equal to the angle enclosed by the pendulum string in its excited position and the stable equilibrium position.
By using Newton's second law of motion and by considering the forces acting on the pendulum it is easy to see that this angle $x(\cdot; g)$ satisfies the parametrised non-linear initial value problem (IVP)
\begin{align*}
  \ddot{x}(\tau; g) &= -\frac{g}{\ell}\sin(x(\tau; g)),\\
  \dot{x}(0; g) &= v_0,\\
  x(0; g) &= x_0,
\end{align*}
where $g$ is the gravitational acceleration of the Earth, $\ell$ denotes the length of the string that connects the two ends of the pendulum, and $\tau \in [0, \infty)$ denotes time. 
An illustration of the model is given in Fig. \ref{Fig_tikz_Pendulum}.

\begin{figure}[h]
  \centering
  \input{sections/FigPendulum}
  \caption{Pendulum model and forces applied to the bob with mass $m$. 
  	The black vertical vector represents the gravitational force. It is decomposed into the gray vectors representing the components parallel and perpendicular to the motion of the pendulum. 
  	The dashed line represents the angle $x=0$ where the pendulum is at rest. In this position the time measurements are taken.}
  \label{Fig_tikz_Pendulum}
\end{figure}

Following the framework presented in \S \ref{Subs_Problem_Form}, we define the model $G(g) = x(\cdot; g)$ which maps the model parameter, here the gravitational acceleration, to the model output, here the time-dependent angle.
For $t  = 1, \dots, 10$ we define the observation operator $\mathcal{O}_t$ by $\mathcal{O}_t(x(\cdot; g)) = x(\tau_t;g)$.
This models the angle measurement of the pendulum at a fixed point in time $\tau_t$.
Note that in practice the measurement is reversed since we measure the time at a prescribed angle that is easy to identify. 
Mathematically, this can be interpreted as angle measurement at a specific timepoint.
Finally, we define the forward response operators $\mathcal{G}_t = \mathcal{O}_t \circ G$ for $t = 1, \dots, 10$.
The data set $y_1, \ldots, y_t$ of angle measurements corresponds to realisations of the random variables
\begin{equation*}
  \widetilde{y}_t := \mathcal{G}_t(g^\dagger) + \eta_t 
\end{equation*}
where $\eta_1, \ldots, \eta_t$ are independent and identically distributed Gaussian random variables according to $N(0, \sigma^2)$.
The pendulum filtering problem consists of using time measurements (and the associated angle measurements) to sequentially improve the estimate of the true value of the Earth's gravitational acceleration $g^\dagger$.
\end{example}

\begin{remark} \label{Remark_linearisedODE}
	It is possible to simplify the mathematical model of the pendulum motion.
	Assume that $v_0 = 0$. If the angle $x$ is small, then $x \approx \sin(x)$. Hence, the nonlinear ODE $\ddot{x}=-(g/\ell) \sin(x)$ above can be replaced by the linear ODE $\ddot{x}=-(g/\ell) x$ with the analytical solution
	\[x(\tau; g) := x_0\cos(\tau\sqrt{g/\ell}).\]
	However, the relation between the angle $x$ and the model parameter $g$ is still nonlinear and thus the filtering problem remains nonlinear with no analytical solution.
	For this reason we do not consider the linear pendulum dynamics.
\end{remark}

\subsection{State of the art}

Model calibration problems have often been approached with optimisation techniques, for example, the Gauss-Newton or Levenberg-Marquardt algorithm. 
These algorithms minimise a (possibly regularised) quadratic loss function which measures the distance between the data and the model output, see e.g. \cite[\S 10]{Noce06}.
Today's availability of high-performance computing resources has enabled statistical techniques for the calibration of computationally expensive models.
A popular example is Bayesian inference.
Here we consider the  model parameters to be uncertain and model the associated uncertainty with a probability measure. 
By using Bayes' formula it is possible to include information from the observational data in this probability measure. 
In particular, the probability measure is conditioned with respect to the data (see \cite{Robert2007}).

Recently, Bayesian inference for model parameters (so-called Bayesian inverse problems) has attracted a lot of attention in the literature. 
It was first proposed in \cite{Kaipio2005} and thoroughly analysed in \cite{Dashti2017,Stuart2010}.
A tutorial on Bayesian inverse problems is given by Allmaras et al. \cite{Allmaras2013}; in fact this work inspired the authors of this article.
However, most works on Bayesian inverse problems, including the works cited above, are concerned with the so-called \emph{static} Bayesian learning where one uses a single set of observations and no filtering is carried out.
Taking the step from including a single set of observations to iteratively including more observations is both practically important and non-trivial.
We mention that the filtering of model parameters is closely related to the filtering of states in state space models.
In the pendulum problem in \S\ref{SubSec_Pendulum} this task corresponds to the tracking and prediction of the pendulum motion.
Filtering of states is a central problem in \emph{data assimilation} (see e.g. \cite{Doucet2011,Law2015,Nakamura2015}).

Linear-Gaussian filtering problems can be solved analytically with the Kalman filter, see e.g. \cite{Humpherys2012}.
For non-linear filtering problems several non-linear approximations to the Kalman filter have been proposed. Examples are the extended Kalman filter (EKF, see e.g. \cite{Humpherys2012}) and the Ensemble Kalman Filter (EnKF, see \cite{Evensen2003}) which are essentially based on linearisations of the forward problem.
The EKF uses a Taylor expansion for linearisation.
The EnKF uses a probabilistic linearisation technique called \emph{Bayes linear} (see e.g. \cite{Latz2016,Schillings2017}).
The Taylor expansion in the EKF can be evaluated analytically, however, for the Bayes linear approximation this is not possible.
For this reason the EnKF uses a particle approximation -- an \emph{ensemble} of unweighted particles.

Another family of approximations, so-called \emph{particle filters}, do not use  linearisation strategies, but rely on importance sampling (see \cite{Robert2004}).
We will discuss two particle filters -- Sequential Importance Sampling and Sequential Monte Carlo -- in this tutorial.
Note that these methods are not only used for filtering.
Indeed, it is possible to sample from general sequences of probability measures by using particle filters.
We refer to \cite{DelMoral2004,DelMoral2013,DelMoral2006} for the theoretical background and further applications of particle filters.
We mention the use of particle filters in static Bayesian inverse problems. 
SMC and SIS are here used together with a tempering of the likelihood (see e.g. \cite{Beskos2016, Beskos2015, Kahle2018, Kantas2014, Neal2001}), with multiple resolutions of the computational model (see e.g. \cite{Beskos2017a}) or with a combination of both (see e.g. \cite{Latz2018}).
Note that SMC requires a Markov kernel that is typically given by a Markov Chain Monte Carlo (MCMC) method \cite{Liu2004, Robert2004}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/2_bayes.tex <==
\section{Bayesian filtering} \label{Sec_Bayes}
In this section we explain the Bayesian approach to the filtering problem discussed in \S\ref{Subs_Problem_Form}.
We begin by introducing conditional probabilities and their construction using Bayes' formula.
We conclude this section by revisiting the pendulum filtering problem in \S\ref{SubSec_Pendulum} and discuss implications from the Bayesian approach.

Consider some uncertain parameter $\theta$.
We model the uncertainty as a random variable; by definition this is a measurable map from the probability space $(\Omega, \mathcal{A}, \mathbb{P})$ to the parameter space $X$.
The probability measure of $\theta$ is called $\mu_0 = \mathbb{P}(\theta \in \cdot)$.
The measure $\mu_0$ reflects the knowledge concerning $\theta$ before we include any information given by observations. 
For this reason $\mu_0$ is called \emph{prior (measure)}.

In \S \ref{Subs_Problem_Form} we modeled the data generation at time $t$ as an event that occurs and that we observe. 
This event is $\{\widetilde{y}_t = y_t\} \in \mathcal{A}$.
The process of \emph{Bayesian learning} consists in including the information ``$\widetilde{y}_t = y_t$'' into the probability distribution of $\theta$.
This is done with conditional probability measures. 
A good intuition about conditional probabilities can be obtained by consideration of discrete probabilities.

\begin{example} \label{Example_CondProb_Disc1}
Let $\theta$ denote a uniformly distributed random variable on the parameter space $X := \{1,\dots,10\}$.
The uniform distribution models the fact that we have no information whatsoever about $\theta$. 
Next, an oracle tells us that ``$\theta$ is about $4$''.
We model this information by assuming that $\theta$ is equal to $3$, $4$ or $5$ with equal probability. 
Our state of knowledge is then modeled by the following conditional probabilities:
\begin{align*}
\mathbb{P}(\theta = k | \theta \text{ is about } 4) := \begin{cases}
1/3, &\text{if } k = 3,4,5, \\
0, &\text{otherwise.}
\end{cases}
\end{align*}
\end{example}
We revisit this example in the next subsection and illustrate the computation of the conditional probability measure.
For now, we move back to the filtering problem. 
Having observed the first data set $y_1$ we replace the prior probability measure $\mu_0$ by the conditional probability measure 
\[
\mu_1 
= 
\mathbb{P}(\theta \in \cdot| \widetilde{y}_1 = y_1).
\]
Analogously to Example \ref{Example_CondProb_Disc1} the measure $\mu_1$ now reflects the knowledge about $\theta$ given the information that the event $\{\widetilde{y}_1 = y_1\}$ occurs.
In the next step we observe $\widetilde{y}_2 = y_2$ and update $\mu_1 \mapsto \mu_2$, where
\[
\mu_2 
= 
\mathbb{P}(\theta \in \cdot| \widetilde{y}_1 = y_1,\, \widetilde{y}_2 = y_2) 
=: 
\mathbb{P}(\theta \in \cdot| \widetilde{y}_{1:2} = y_{1:2}).
\]
This update models the Bayesian filtering from time point $t=1$ to $t=2$.
More generally, we can define a Bayesian filter as a map
 \[
 \{\mu_t, y_{t+1}\} 
 :=  
 \{\mathbb{P}(\theta \in \cdot| \widetilde{y}_{1:t} = y_{1:t}), y_{t+1}\}\mapsto \mathbb{P}(\theta \in \cdot| \widetilde{y}_{1:t+1} = y_{1:t+1})
  =:
  \mu_{t+1}.
 \]
Since $\mu_t$ reflects the knowledge about $\theta$ after seeing data, this measure is called \emph{posterior (measure) at time $t$} for every $t \geq 1$.
The notions and explanations in \S \ref{Subs_Problem_Form} can be transferred to Bayesian filtering by replacing $\widehat{\theta}(y_{1:t})$ with $\mu_t$.

\subsection{Bayes' formula} \label{Subs_Bayes_Form}
The Bayesian learning procedure -- formalised by the map $\{\mu_t, y_{t+1}\} \mapsto \mu_{t+1}$ -- is fundamentally based on Bayes' formula.
In order to define Bayes' formula, we  make some simplifying, yet not necessarily restrictive assumptions.

In \S \ref{Subs_Problem_Form} the parameter space $X$ can be infinite-dimensional. 
In the remainder of this tutorial we consider $X:= \mathbb{R}^N$, a finite-dimensional parameter space.
For a treatment of the infinite dimensional case we refer to \cite{Stuart2010}. 
Moreover, we assume that $\mu_0$ has a \emph{probability  density function (pdf)} $\pi_0: X \rightarrow \mathbb{R}$ with respect to the Lebesgue measure. 
This allows us to represent $\mu_0$ by $$\mu_0(A) := \int_A \pi_0(\theta) \mathrm{d}\theta,$$
for any measurable set $A \subseteq X$.
Furthermore, we assume that the \emph{model evidence}
\begin{align*}
{Z_{t+1}(y_{t+1})} 
&:= 
\mu_t\left(L_{t+1}(y_{t+1}|\cdot)\right)  
:= 
\int_X L_{t+1}(y_{t+1}|\theta)  \mathrm{d}\mu_t(\theta)\\ 
&:= 
\int_X L_{t+1}(y_{t+1}|\theta) \pi_t(\theta)  \mathrm{d}\theta, \quad t \geq 0,
\end{align*}
is strictly positive and finite. 
Then it follows that the conditional measures $\mu_1, \mu_2,\dots$ have pdfs $\pi_1, \pi_2,\dots$ on $X$ as well. 
The associated densities are given recursively by \emph{Bayes' formula}
\begin{equation}\label{Eq_Bayes_Formula}
\pi_{t+1}(\theta) 
= 
\frac{1}{Z_{t+1}(y_{t+1})} L_{t+1}(y_{t+1}|\theta) \pi_t(\theta),  \quad t \geq 0,  \quad \text{a.e. }\theta \in X.
\end{equation}
In some situations it is possible to use this formula to compute the densities $(\pi_t)_{t=1}^\infty$ analytically. In particular, this is possible if  $\pi_t$ is the pdf of a \emph{conjugate prior} for the likelihood $L_{t+1}$ for $t \geq 0$.
However, in the filtering of parameters of nonlinear models it is typically impossible to find conjugate priors. 
In this case we construct approximations to the densities $(\pi_t)_{t=1}^\infty$ and the measures $(\mu_t)_{t=1}^\infty$, respectively.
We discuss particle based approximations in \S \ref{Sec_SMC}.

Before moving on to the Bayesian formulation of the pendulum filtering problem, we briefly revisit Example \ref{Example_CondProb_Disc1} and explain Bayes' formula in this setting.
Note that Bayes' formula holds more generally for probability density functions that are given w.r.t. to $\sigma$-finite measures, for example, \emph{counting densities} on $\mathbb{Z}$; these are sometimes called \emph{probability mass functions (pmf)}.

\begin{example}
Recall that we consider a uniformly distributed random variable $\theta$ taking values in $\{1,\dots,10\}$. 
Hence the counting density is given by $\pi_0 \equiv 1/10$.
Furthermore, an oracle tells us that ``$\theta$ is about 4'' and we model this information by $\theta$ takes on values in $\{3,4,5\}$ with equal probability.
Hence
$$
L_1(y_1|k) 
= 
\mathbb{P}(\theta \text{ is about } 4 | \theta = k ) = \begin{cases}
1, &\text{ if } k = 3,4,5,\\
0, &\text{ otherwise.}
\end{cases}
$$
Now we compute the posterior counting density using Bayes' formula.
We arrive at
\begin{align*}
\pi_1(k) &= \frac{1}{Z_1(y_1)} \cdot \pi_0(k)  \cdot L_1(y_1|k) \\&=  \begin{cases}
\frac{1}{1\cdot\frac{1}{10}+1\cdot\frac{1}{10}+1\cdot\frac{1}{10}} \cdot \frac{1}{10} \cdot 1, &\text{ if } k = 3,4,5,\\
0, &\text{ otherwise.}
\end{cases}
\\
&=  \begin{cases}
1/3, &\text{ if } k = 3,4,5,\\
0, &\text{ otherwise.}
\end{cases}
\end{align*}
Moreover, the values of counting densities are identical to the probability of the respective singleton. 
Thus,  $\pi_1(k):= \mathbb{P}(\theta = k |\theta \text{ is about } 4)$.
Hence the intuition discussed in Example \ref{Example_CondProb_Disc1} was correct.
\end{example}




\subsection{Bayesian filtering formulation of the pendulum problem} \label{Subsec_Bayesian_Pendulum_formulation}
Next, we revisit the pendulum filtering problem in \S\ref{SubSec_Pendulum}, and reformulate it as a Bayesian filtering problem. 
This requires to define a prior measure for the parameter $g$.
The prior should include all information about the parameter before any observations are made.
The first piece of information about $g$ stems from the physical model which describes the motion of  the pendulum. 
Indeed, since we know that gravity attracts objects towards the center of the Earth, we conclude that the value of $g$ must be non-negative in the coordinate system we use. 
Furthermore, we assume that previous experiments and theoretical considerations tell us that $g \le 20m/s^2$, and that $g$ is probably close to the center of the interval $[0, 20]$. 
We model this information by a normal distribution with unit variance, centered at $10$, and truncated support on the interval $[0, 20]$.
Thus, the prior density is proportional to 
\[
 \pi_0(g) 
 \propto 
 \begin{cases} \exp\left(-\frac{1}{2}(g-10)^2\right), &0 \leq g \leq 20, \\
0, &\text{ otherwise.}
\end{cases}
\]
Furthermore, the data generating distribution in \S\ref{SubSec_Pendulum} implies that the likelihoods are given by
\begin{equation}\label{Eq_Pendulum_Likelihoods}
  L_t(y_t|g)
  \propto \exp\left(-\frac{1}{2\sigma^2}\left(y_t - \mathcal{G}_t(g)\right)^2\right), \quad t=1,\dots,10,
  \end{equation}
  where $\sigma^2$ denotes the noise variance. 
  Existing studies (see \cite{thorpe1996speed}) suggest that a typical visual reaction time for humans is of approximately $450\text{ms} \pm 100\text{ms}$. We now would like to use this information about error in the time measurements for modelling the error in the angles. To do this, we use the forward model parameterised by the mean of the prior distribution to compute a reference solution for a set of generated time measurements. We then compute a Monte Carlo estimate of the angle error resulting from adding a $N(0.45, 0.01)$ noise to the set of time measurements. The result of this numerical experiment indicates that $N(0, \sigma^2)$ with $\sigma^2 = 2.5\mathrm{e}{-3}$ is a suitable model of the angle measurements error.

By inserting the prior density and the definition of the likelihoods into Bayes' formula \eqref{Eq_Bayes_Formula} we obtain a recursive expression for the densities $\pi_1, \ldots, \pi_{10}$ of the posterior measures $\mu_1, \ldots, \mu_{10}$ as follows:
\begin{align*}
\pi_{t+1}(g) 
&:= 
\frac{1}{Z_{t+1}(y_{t+1})} \exp\left(-\frac{1}{2\sigma^2}\left(y_t - \mathcal{G}_t(g)\right)^2\right) \pi_t(g), \ \ \text{for a.e. }g \in [0,20],\\
Z_{t+1}(y_{t+1}) &:= \mu_{t+1}\left(\exp\left(-\frac{1}{2\sigma^2}\left(y_t - \mathcal{G}_t(g)\right)^2\right)\right),   \ \ t \geq 0.
\end{align*}
 The family of posterior densities is depicted in Fig.~\ref{Fig_Im_Densities}.  
 As the time increases we see that the posterior densities becomes more concentrated around the true value $g^\dagger \approx 9.81m/s^2$.
 Note that a more concentrated density indicates less uncertainty compared to a flat density.
Thus, the picture is consistent with our intuition: The uncertainty in the parameter value for $g$ is reduced as more data becomes available.
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.5]{posteriors_densities}
  \caption{Sequence of posterior densities for a given value of $g$ for $t = 0\ (\text{prior}), 4, 8, 10$ data points. 
  The densities are computed with kernel density estimation based on a Sequential Monte Carlo particle approximation.
 }
  \label{Fig_Im_Densities}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/3_smc.tex <==
\section{Particle filters} \label{Sec_SMC}

It is typically impossible to compute the posterior measures $(\mu_t)_{t=1}^\infty$ analytically.
In this section we discuss two particle filters to approximate the solution of the Bayesian filtering problem. 
%the \emph{Sequential Monte Carlo} (SMC) algorithm to approximate the solution of the Bayesian filtering problem.  
In \S \ref{Subs_SIS} we present the \emph{Sequential Importance Sampling} (SIS) algorithm. %, which serves as basis for the construction of the SMC algorithm. 
Unfortunately, SIS suffers from efficiency issues when used for filtering problems.
We explain this deficiency in a simple example.
It is possible to resolve the issues by extending SIS to the so-called \emph{Sequential Monte Carlo} (SMC) algorithm which we discuss in \S \ref{Subs_SMC}.
%These issues can be solved by extending SIS can to the SMC algorithm.
%We discuss this extension in \S \ref{Subs_SMC}.
We conclude in \S \ref{Subs_Num_Pendulum} by applying the particle filters to the pendulum filtering problem in \S \ref{SubSec_Pendulum}.

\begin{remark}
The sampling procedures presented in this section approximate posterior measures $(\mu_t)_{t= 1}^\infty$.
In addition, it is also possible to approximate integrals of the form $(\mu_t(f))_{t= 1}^\infty$, where $f: X \rightarrow \mathbb{R}$ is a $\mu_t$-integrable \emph{quantity of interest}.
To simplify the presentation we focus on the approximation of integrals rather than on the approximation of measures for the remaining part of this tutorial.
This can be done without loss of generality within the framework of weak representations of measures.
We outline this approach and give some examples for quantities of interest in Appendix A.
\end{remark}

\subsection{Sequential Importance Sampling}\label{Subs_SIS}

We are now interested in constructing an algorithm to approximate the sequence of posterior measures $(\mu_t)_{t=1}^\infty$ and thereby efficiently discretise the update rule of the learning process in Fig. \ref{Fig_tikz_learning}. 
To this end we consider \emph{particle-based} approximations.
These consist of a collection of $M$ weighted \emph{particles} (or \emph{samples}) $\{X_i, W_i\}_{i=1}^M$ where $X_i \in X$, $W_i \ge 0$ for $i = 1, \ldots, M$, and $\sum_{i=1}^MW_i = 1$. 
Additionally, the particles should be constructed in such a way that the \emph{random measure} $$\mu^M_t := \sum_{i=1}^MW_i\delta_{X_i}$$ converges \emph{weakly with probability one} to $\mu_t$ as $M \rightarrow \infty$. 
In particular, for any  bounded and continuous function $f : X \rightarrow \mathbb{R}$ (or bounded and Lipschitz-continuous function; see Prop. \ref{Prop_Convergence} in Appendix A),
\begin{align*}
  \mu_t^M(f) := \sum_{i=1}^MW_if(X_i) \xrightarrow{M \rightarrow\ \infty}  \mathbb{E}[f(\widehat\theta_t)] && \text{almost surely.}
\end{align*}
Note that $(\mu_t^M)_{M \geq 1}$ is a sequence of measure-valued random variables; that is a sequence of random variables defined on the space of measures. 
Almost every realisation of this sequence of measures converges weakly to a common deterministic measure as $M \rightarrow \infty$. 
More precisely, it holds that $$\mathbb{P}(\mu_t^M\rightarrow \mu_t, \text{ weakly, as }M \rightarrow \infty) = 1.$$

For simple distributions $\mu$ where direct sampling is possible an estimator with the desired properties above can be constructed by choosing independent random variables $X_1, \ldots, X_M$ distributed according to $\mu$ and by using uniform weights $W_i = 1/M$ for $i = 1, \ldots, M$. 
We denote this construction by the operator $S^M$ and call $\mu^M = S^M\mu$ the \emph{standard Monte Carlo} estimate of $\mu$. 
Since $S^M$ creates an empirical measure by using random variables the operator $S^M$ maps probability measures to random probability measures and is thus a non-deterministic operator.

However, it is typically impossible to sample from the posterior measures $(\mu_t)_{t=1}^\infty$ in the Bayesian filtering problem.
This precludes the construction of Monte Carlo estimates. 
Alternatively, we can use the \emph{Importance Sampling} (IS) method.
Let $\mu$, the \emph{target measure}, denote the probability measure to be estimated.
Let $\nu$ denote a probability measure from which it is possible to sample.
The measure $\nu$ is called \emph{importance measure}. 
Let $\mu$ be \emph{absolutely continuous} with respect to $\nu$.
This means that $\nu(A) = 0$ implies $\mu(A) = 0$ for any measurable set $A \subseteq X$.
Let furthermore $f$ denote a measurable, bounded function.
Then there exists a non-negative function $w : X \rightarrow \mathbb{R}$ such that
\begin{equation}\label{Eq_Radon_Nikodym}
  \mu(f) = \frac{\nu(f \cdot w)}{\nu(w)}.
\end{equation}
The intuition behind importance sampling is the following.
If the importance measure $\nu$ is close to the target measure $\mu$, then sampling from $\nu$ should be approximately equivalent to sampling from $\mu$. 

The IS estimate of $\mu$ is constructed by creating a Monte Carlo estimate of $\nu$.
Then, the Monte Carlo samples are reweighed using the expression in \eqref{Eq_Radon_Nikodym}.
This is necessary since we wish to obtain samples distributed according to the target measure $\mu$, and not samples distributed according to the importance measure $\nu$.
We arrive at
\begin{equation*}
  \mu^M(f)
  = 
  \frac{\nu^M(f \cdot w)}{\nu^M(w)} 
  = 
  \frac{\frac1M\sum_{i=1}^Mw(X_i)f(X_i)}{\frac1M\sum_{j=1}^Mw(X_j)} 
  :=
  \sum_{i=1}^MW_if(X_i).
\end{equation*}
In summary, importance sampling maps the Monte Carlo estimate $\nu^M$ to an updated estimate $\mu^M$ by adjusting the weights of the particles $X_1, \ldots, X_M$ according to the formula
\begin{equation*}
  W_i = \frac{w(X_i)}{\sum_{j=1}^Mw(X_j)}.
\end{equation*}

Now we apply the IS approximation in the context of the Bayesian filtering problem.
The prior measure $\mu_0$ is often tractable and direct sampling algorithms are available. 
It is then possible to create an initial Monte Carlo estimate of the prior measure.
Afterwards we can iteratively update the particles to incorporate the new knowledge from the observation $y_1, y_2, \ldots, y_T$ through importance sampling.
This follows the learning process described in \S \ref{Subs_Problem_Form}. 
Observe that Bayes' formula in \eqref{Eq_Bayes_Formula} tells us that each measure $\mu_{t+1}$ is absolutely continuous with respect to the previous measure.
We use this relation to define the nonlinear operator $\is_t$ for any probability measure $\mu$ over $X$ as follows:
\begin{equation*}
  (\is_{t+1} \mu)(f) 
  = 
  \frac{\mu(L_{t+1}(y_{t+1} | \cdot) \cdot f)}{\mu(L_{t+1}(y_{t+1} | \cdot))}.
\end{equation*}
Since $Z(y_{t+1}) = \mu_t(L_{t+1}(y_{t+1} | \cdot))$ for every $t \ge 0$ these operators can be used describe reweighing in an importance sampling estimate with target measure $\mu_{t+1}$ and importance measure $\mu_t$. 
In particular, if for some $t \ge 0$ a particle approximation $\mu_t^M$ of $\mu_t$ is given by the particles $\{X^{(t)}_i, W^{(t)}_i\}$, the operator $\is_{t+1}$ can be used to define the following approximations:
\begin{align*}
  Z^M(y_{t+1}) &:= \mu_t^M(L_{t+1}(y_{t+1} | \cdot)) = \sum_{i=1}^MW^{(t)}_iL_{t+1}(y_{t+1} | X_i),\\
  \mu_{t+1}^M(f) &:= (\is_{t+1} \mu_t^M)(f) \\ &= \frac1{Z^M(y_{t+1})}\sum_{i=1}^MW^{(t)}_iL_{t+1}(y_{t+1} | X^{(t)}_i)f({X^{(t)}_i}) \\ &= \sum_{i=1}^MW^{(t+1)}_if({X^{(t)}_i}),
\end{align*}
where the particle weights $W^{(t+1)}_i$ are given by
\begin{equation*}
  W^{(t+1)}_i = \frac{W^{(t)}_iL_{t+1}(y_{t+1} | X^{(t)}_i)}{\sum_{j=1}^MW_j^{(t)}L_{t+1}(y_{t+1} | X_j^{(t)})}.
\end{equation*}
Note that the $\is_{t+1}$ update requires $\sum_{j=1}^MW_j^{(t)}L_{t+1}(y_{t+1} | X_j^{(t)}) > 0$. 
If the likelihood $L_{t+1}(y_{t+1} | \cdot )$ is strictly positive, then this condition is always satisfied.
We observe that the IS update formula only changes the weights $$(W_i^{(t)})_{i=1}^M \mapsto (W_i^{(t+1)})_{i=1}^M.$$ 
The positions $(X_i^{(t)})_{i=1}^M = (X_i^{(t+1)})_{i=1}^M$ of the particles remain unchanged.
Based on the recursive update formula, we construct an approximation to the sequence $(\mu_t)_{t=0}^\infty$ as follows:
\begin{align*}
\mu_0^M &= S^M\mu_0, \\
\mu_{t+1}^M &= \is_{t+1}(\mu_t^M).
\end{align*}

\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.6]
  \draw	(1.5,0)node[anchor=east] {timeline:};
  \draw	(1.5,-1)node[anchor=east] {state of knowledge:};
  
  \draw	(3,0.35)node[align=center] {$t$};
  \draw	(9,0.35)node[align=center] {$t+1$};
  \draw	(15,0.35)node[align=center] {$t+2$};

  \draw[line width = 1.0, color = black,-](3,0.1) -- (3,-0.1);
  \draw[line width = 1.0, color = black,-](9,0.1) -- (9,-0.1);
  \draw[line width = 1.0, color = black,-](15,0.1) -- (15,-0.1);
  
  \draw[line width = 1.5, color = black,->](6.5,-1) -- (11.7,-1);
  \draw[line width = 1.0, color = black,->](2,0) -- (16.5,0);
  
  \draw	(4.25,-1)node[rectangle,anchor=west,text width=0.75cm, thick,draw=black,align=center,fill=white] {$\mu_t^M$};
  
  \draw[line width = 1.5, color = black,<-](9,-1.65) -- (9,-2.5);
  \draw	(9,-3)node[align=center] {$y_{t+1}$};

  \draw	(7,-1)node[align=center,rectangle,anchor=west,thick,draw=black,fill=white] {Reweigh by $\is_{t+1}$};

  \draw	(12.05,-1)node[align=center,rectangle,anchor=west,text width=0.75cm,thick,draw=black,fill=white] {$\mu_{t+1}^M$};
 \end{tikzpicture}
 \caption{Plot of the SIS approximation of the learning procedure. 
 The starting point is the approximation $\mu_t^M$ of the current state of knowledge at timepoint $t$. 
 At the timepoint $t+1$ we observe $y_{t+1}$ and use it to construct the importance sampling operator $\is_{t+1}$. 
 The new state of knowledge is approximated by $\mu_{t+1}^M$. }
\label{Fig_tikz_learning_sis}
\end{figure}
The sequential importance sampling algorithm is a natural and asymptotically correct approximation of the Bayesian filtering process, see e.g. \cite{Beskos2015,Bulte2018} for up to a finite number of observations. %, see Example \ref{Example_Gaussian_degeneracy}.
Now we discuss the accuracy of (sequential) importance sampling measured in terms of the so-called \emph{effective sample size (ESS)}.
Let $t \geq 0$. 
First, we define the constant $\rho_t > 0$ by
\begin{equation*}
  \rho_t := \frac{\mu_0(\mathbf{L}_t^2)}{\mu_0(\mathbf{L}_t)^2},
\end{equation*}
where $\mathbf{L}_t(\theta) = \prod_{i=1}^t L(y_t|\theta)$ is the joint likelihood of the dataset $y_{1:t}$.
One can show that the accuracy of (sequential) importance sampling up to time $t$ is equivalent to the accuracy of a standard Monte Carlo approximation with $M/\rho_t$ samples (see e.g. \cite{Agapiou2015}).
The fraction $M/\rho_t$ is the {effective sample size}.
The ESS can be interpreted as follows.
\begin{enumerate}
\item If $M/\rho_t \approx M$, then the estimation is (almost) as accurate as sampling directly from the correct measure.
\item If $M/\rho_t \ll M$, then the estimation is only as accurate as a Monte Carlo approximation with a very small number of particles.
\end{enumerate}
Unfortunately, during the course of a filtering procedure, it may happen that $\rho_t$ explodes. 
We illustrate this by a simple example.
\begin{example} \label{Example_Gaussian_degeneracy}
Consider the problem of estimating the mean $m^\dagger$ of a normal distribution $\mathrm{N}(m^\dagger, 1)$ using $t \in \mathbb{N}$ samples $y_1, \ldots, y_t$ of the distribution. 
By choosing the conjugate prior $\mathrm{N}(0, 1)$ it is easy to see that the posterior distribution of the unknown parameter $m$ is equal to $\mathrm{N}\left(\frac{S_t}{t+1}, (1 + t)^{-1}\right)$, where $S_t = \sum_{i=1}^ty_i$. 
It is possible to compute $\rho_t$ analytically.
We obtain
  \begin{equation*}
    \rho_t = \frac{t+1}{\sqrt{2t+1}}\exp\left(\frac{S_t^2}{(2t+1)(t+1)}\right).
  \end{equation*}
  Hence, $\rho_t = O(t^{1/2}; t \rightarrow \infty)$ grow unboundedly as $t$ increases.
  This implies that the effective sample size $M/\rho_t$ converges to $0$ as $t\rightarrow \infty$.  
\end{example}
In a filtering problem where $M/\rho_t \rightarrow 0$ as $t\rightarrow \infty$ we cannot use SIS since the estimate deteriorates over time.
It is possible, however, to estimate the effective sample size, and to use this estimate to improve SIS.

\subsection{Sequential Monte Carlo}\label{Subs_SMC}
The effective sample size is a good indicator of the impoverishment of the particle estimate for $\mu_t$ due to the discrepancy between the importance and target distributions. 
%We aim to use the information provided by it to improve our algorithm.
In practice, we approximate $M/\rho_t$ by 
\begin{equation} \label{Eq_Ess_Approx_Sec_Moment}
  \ess 
  :=  
  M\frac{\mu_0^M(\mathbf{L}_t)^2}{\mu_0^M(\mathbf{L}_t^2)}
  =
  \frac{\left(\sum_{i=1}^M \mathbf{L}_{t}(X_i)\right)^2}{\sum_{i=1}^M \mathbf{L}_{t}(X_i)^2}.
\end{equation}
Note that $\ess$ is a consistent estimator of $M/\rho_t$.
Throughout the rest of this tutorial we will also refer to $\ess$ as \emph{effective sample size}.

If $\ess$ is small it is possible to discard particles situated in regions of the parameter space with low probability.
We can then replace these particles with particles that are more representative of the target distribution in the sense that they carry a larger weight.
This is done by introducing a \emph{resampling step} after adjusting the weights of the particles in the IS estimate. 
Precisely, we consider an approximation $\mu_t^M$ given by the particles $\{X_i^{(t)}, W_i^{(t)}\}_{i=1}^M$ at time $t\geq 0$. 
The weights of the approximation are updated by the $\is_{t+1}$ operator, and $\ess$ is computed using the updated set of weights $(W_i^{(t+1)})_{i=1}^M$. 
If $\ess$ is larger than a pre-defined threshold $\mlow \in (0, M)$, then the positions of the particles remain unchanged in the step from $\mu_t^M$ to $\mu_{t+1}^M$, giving $X_i^{(t+1)} = X_i^{(t)}, i=1,\dots,M$. 
If, on the other hand, it holds $\ess \le \mlow$, then a new set of particles is sampled according to the updated weights.
The particle estimate is then given by $\mu_{t+1}^M = S^M(\is_{t+1}\mu_t^M)$ where we use the new particle set in the Monte Carlo estimate.

The resampling procedure can be performed as follows.
For $i=1,\dots,M$ sample $U_i \sim \mathrm{Unif}[0,1]$, a uniform random variable between $0$ and $1$.
Then, define
\begin{align*}
X_i^{(t+1)} &:= X_j^{(t)},\ \ j = \min\left\lbrace k \in \{1,\dots,M\} :\sum_{n=1}^k W_n^{(t+1)} \geq U_i \right\rbrace, \\
W_i^{(t+1)} &:= 1/M.
\end{align*}
Alternative ways of resampling are possible (see \cite{Gerber2017}).
Note that the resampling step can successfully eliminate particles in low density areas of the parameter space.
However, it still fails to reduce the particle degeneracy, since several particles may occur in the same position. 
Moreover, even  with resampling the particles cannot fully explore the parameter space, since their position remains fixed at all times. 

Due to the resampling in case of a small value $\ess$ or if $\ess$ is large, it is reasonable to assume that the remaining particles are approximately $\mu_{t+1}$-distributed.
The idea is now to scatter the particles in a way such that they explore the parameter space to reduce degeneracy without destroying the approximate $\mu_{t+1}$-distribution.
This can be achieved by a scattering with $\mu_{t+1}$-invariant dynamic.
Such a dynamic is given by an ergodic Markov kernel
$K_{t+1} : X \times \mathcal{B}(X) \rightarrow [0, 1]$  that has $\mu_{t+1}$ as stationary distribution.
This means if $X \sim \mu_{t+1}$ and $X' \sim K(X, \cdot)$, then $X' \sim \mu_{t+1}$.
Applying the Markov kernel repeatedly to a single particle will asymptotically produce particles that are $\mu_{t+1}$ distributed independently of the initial value (see \cite[Chapter~6]{Robert2004}).
Since we assumed that the particles are  approximately $\mu_{t+1}$-distributed, we typically rely only weakly on this asymptotic result.

\begin{figure}[t!]
  \centering
  \input{sections/FigSMC}
  \caption{Plot of the SMC approximation of the learning procedure. 
  The approximation is constructed in three steps: \emph{reweighing} to identify representative particles, \emph{resampling} to discard particles in low probability regions, and a \emph{correction} to adjust the position of the particles to the new state of knowledge. }
\label{Fig_tikz_learning_smc}
\end{figure}

The reader might find it not easy to construct an ergodic Markov kernel $K_t$ that has $\mu_t$ as a stationary measure, $t \geq 1$.
However, this is a standard task in so-called Markov Chain Monte Carlo methods (MCMC).
The literature on MCMC offers a large variety of suitable Markov kernels.
We mention Gibbs samplers, Hamiltonian Monte Carlo Metropolis--Hastings, Random--Walk--Metropolis, Slice samplers (see e.g. \cite{Liu2004,Robert2004}).
Thus we add a final step to the approximation, and apply once or several times the transition kernel $K_t$ to each of the particles to obtain a better coverage of the probability density of the posterior at time $t$. 
The resulting algorithm is the \emph{Sequential Monte Carlo} (SMC) method.
Its approximation of the learning process is depicted in Fig.~\ref{Fig_tikz_learning_smc}.

\section{Particle approximation of the Bayesian pendulum filtering} \label{Subs_Num_Pendulum}

We are now ready to compute an approximate solution to the Bayesian filtering problem in \S \ref{Subsec_Bayesian_Pendulum_formulation}. 
To this end we consider the likelihoods in \eqref{Eq_Pendulum_Likelihoods} and use the  set of measurements given in Table~\ref{Table_measurements}. 


%\begin{table}[h]
%  \begin{center}
%    \begin{tabular}{|c|c|c|}
%      \hline 1 & 10.04 $\pm$ 0.119 & 9.939 $\pm$ 0.109 \\
%      \hline 2 & 10.08 $\pm$ 0.090 & 9.978 $\pm$ 0.049 \\
%      \hline 3 & 10.05 $\pm$ 0.050 & 10.02 $\pm$ 0.054 \\
%      \hline 4 & 9.973 $\pm$ 0.028 & 10.00 $\pm$ 0.025 \\
%      \hline 5 & 9.998 $\pm$ 0.026 & 10.00 $\pm$ 0.024 \\
%      \hline 6 & 10.02 $\pm$ 0.016 & 10.02 $\pm$ 0.013 \\
%      \hline 7 & 9.999 $\pm$ 0.012 & 9.999 $\pm$ 0.009 \\
%      \hline 8 & 9.912 $\pm$ 0.008 & 9.898 $\pm$ 0.007 \\
%      \hline 9 & 9.877 $\pm$ 0.007 & 9.872 $\pm$ 0.005 \\
%      \hline 10 & 9.791 $\pm$ 0.006 & 9.803 $\pm$ 0.003 \\
%      \hline
%      \end{tabular}
%  \end{center}
%\end{table}
%
\begin{table}[h]
  \begin{center}
    \begin{tabular}{|l r|r r r r r r r r r r|}
      \hline measurement & $t$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & ${10}$  \\
      \hline
  time & $\tau_t$ &  1.51s & 4.06s & 7.06s & 9.90s & 12.66s & 15.40s & 15.58s & 18.56s & 21.38s & 24.36s \\ 
% angle &  $y_t$ &  0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
      \hline
    \end{tabular}
  \end{center}
  \caption{Time measurements corresponding to the angle $x=0$ of a simple pendulum.}
  \label{Table_measurements}
\end{table}
These measurements have been collected from a pendulum with length $\ell := 7.4m$.
The initial angle $x_0 = 5^\circ = \pi/36$, and the initial speed $v_0 = 0$. 
Since $x_0$ is small and $v_0 = 0$, it would be possible to consider the linearised IVP with an analytical solution (see Remark \ref{Remark_linearisedODE}).
In tests not reported here the filtering solution obtained with the analytical solution of the linearised IVP did not differ from the numerical solution of the nonlinear IVP.\medskip

\lstinputlisting[caption={Python file {\fontfamily{txtt}\selectfont smc\_approx.py}.},captionpos=b,label=lst:python]{figures/smc_code.py}

The numerical results presented in the following sections have been computed with {\sc Python}.  
The associated Python code is available online \todo{link to github repo}, and a part of the code is printed in display \todo{put reference here}.
It can be combined with the data set of time measurements in Table\ref{Table_measurements} to reproduce our results, and to carry out further experiments.
The code in Display \ref{lst:python} also summarises the complete modelling cycle of the pendulum filtering problem.


\subsubsection{SIS}
We first construct approximations of the learning process using the SIS algorithm as illustrated in Fig. \ref{Fig_tikz_learning_sis}. 
We employ different numbers of particles, $M = 2^4,2^5,\dots,2^{12}$, and perform 50 simulations for each value of $M$.
%In each of these settings, we consider results of $20$ simulations.
In Fig. \ref{Fig_Im_SIS} we present the results of the SIS approximations of the posterior distribution at time $t = 10$ depending on the number of particles $M$.
\begin{figure}[h]
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{sis_mean_convergence}
  \end{minipage}
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{sis_asymptotic_variance_convergence}
  \end{minipage}
  \caption{Accuracy of the SIS approximation. 
  	In the plots we use data from runs with a variable number of particles indicated on the horizontal axis. We show results averaged over 50 runs per setting. Left: Plot displaying the convergence of the estimated mean of the posterior distribution. Each black dot represents the sample average over $50$ runs, and the bars represent the standard deviation of the mean within the runs. Right: Plot displaying the asymptotic convergence of the variance of the posterior mean estimate.}

  \label{Fig_Im_SIS}
\end{figure}
The left display in this figure shows that the variance of the posterior mean estimate is reduced as the number of particles $M$ is increased.
Moreover, we observe in the right display of the figure that the convergence rate of the variance of the posterior mean estimate is $O(1/M)$.
This coincides with the rate of a standard Monte Carlo approximation and is expected \todo{put reference here}.
Hence, we conclude that the SIS estimate converges as $M \rightarrow \infty$.

Next, we fix the number of particles $M = 2500$, and investigate the accuracy in the SIS approximation by studying the effective sample size. 
Anticipated by the plot of the densities in Fig. \ref{Fig_Im_Densities} and by Example \ref{Example_Gaussian_degeneracy} we expect that the prior distribution is a poor importance distribution for the sequence of posterior distributions constructed during the learning process. 
This intuition is confirmed by numerical experiments shown in Fig. \ref{Fig_Im_SIS_Run} where we see that the effective sample size decreases until it is under $50\%$ of the intial sample size.

\begin{figure}[h]
  \centering
  \begin{minipage}{.5\textwidth}
  \includegraphics[width=\linewidth]{sis_ess}
  \end{minipage}
  \caption{Plot of the effective sample size for the SIS approximation of the learning process. 
  	As the number of observations increases the prior distribution is an increasingly poor importance distribution for the updated posteriors. This is consistent with the fast reduction of the effective sample size over time; implying a loss of estimator accuracy over time. }
  \label{Fig_Im_SIS_Run}
\end{figure}

Recall that the mean square error of a Monte Carlo estimator with $20\% \cdot M$ samples is 5 times larger compared to the mean square error with $M$ samples. 
In the simple pendulum setting, where the parameter space space is one dimensional and compact, a sample size of $50\% \cdot M$ is likely still sufficient to obtain a useful posterior estimate. 
Indeed, the estimation results with SIS do not differ significantly from the estimation results with SMC.
In real-world applications, however, we typically encounter high-dimensional and unbounded parameter spaces which require the exploration with a large number of representative samples.
In this case, the decrease of the effective sample size in SIS is a serious drawback. 
%Therefore, we proceed with an SMC approximation of the pendulum filtering problem.
\begin{figure}[!t]
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_typical_density}
  \end{minipage}
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_typical_ess}
  \end{minipage}
  \caption{SMC approximation of the final posterior distribution of the learning process at $t = 10$. 
  	Left: Histogram of the estimated measure $\mu_{10}$ computed by the particle approximation. 
  	Right: Plot of the effective sample size over time. 
  	Since $\mlow=1875$ the SMC algorithm performed $3$ resampling steps to maintain a large effective sample size.  }
  \label{Fig_Im_Typical}
\end{figure}

\subsubsection{SMC} \label{Subsubsec_SMC}
We proceed by constructing an approximation of the learning process using the SMC algorithm. 
The Markov kernel $K_t$ is given by a Random-Walk-Metropolis algorithm with target distribution $\mu_t$ and a Gaussian random walk \textcolor{red}{with standard deviation $0.25$} as proposal distribution.
Each Markov kernel $K_t$ is applied $5$ times to correct the approximated distribution.
We choose a minimal effective sample size corresponding to $75\%$ of the total population $M$.
This means that we resample, if $\ess < \mlow := 75\% \cdot M$. 

We present a typical run of the algorithm in Fig. \ref{Fig_Im_Typical}.
Again $M = 2500$ particles are used to approximate the learning procedure.
In Fig. \ref{Fig_Im_Typical} we see that the SMC approximation to the posterior measure for $t=10$ is centered around the true value $g^\dagger \approx 9.81 m/s^2$. 
Moreover, we see that 3 resampling steps have been performed.
This maintains an ESS well over $1600$ and thus improves the accuracy of the posterior estimate with SMC compared to the estimate with SIS.

To validate the SMC posterior estimate of $\mu_{10}$ with $M = 2500$ particles, we have performed a reference run using a Markov chain Monte Carlo sampler.
The MCMC sampler was run with 3000 posterior samples where the first 500 samples have been discarded to mitigate the burn-in effect.
Using the MCMC and SMC samples we perform a kernel density estimation for the posterior pdf.
We present the estimation results in Fig. \ref{Fig_SMCMCMC}.
The posterior approximations do not differ significantly which leads us to conclude that the SMC approximation is consistent with the MCMC approximation.

\begin{figure}[!t]
\centering
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_mcmc_kernel_densities.png}
  \end{minipage}
  \caption{Kernel density estimates of $\mu_{10}$ using the MCMC reference solution and the SMC solution. Each estimate is based on 2500 samples.}  
  \label{Fig_SMCMCMC}
\end{figure}

Moreover, we again investigate the convergence of SMC based on simulations with different numbers of particles  $M = 2^4,2^5,\dots,2^{12}$.
In each of these settings we consider the results of $50$ simulations.
We present the test results in Fig. \ref{Fig_Im_SMC}.
We plot the posterior mean approximation at time $t = 10$ and the variance of the estimators within 50 simulations.
\begin{figure}[h]
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_mean_convergence}
  \end{minipage}
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_asymptotic_variance_convergence}
  \end{minipage}
  \caption{Accuracy of the SMC approximation. 
  In theplots we use data from runs of the SMC algorithm with a variable number of particles indicated on the horizontal axis of each plot. 
  We show results averaged over 50 runs per setting.  
  Left: Plot displaying the convergence of the estimated mean of the posterior distribution. 
  The black dots represent the average over $50$ runs and the bars represent the standard deviation of the mean within the runs. 
  Right: Plot displaying the convergence of the variance of the posterior mean estimate.}
  \label{Fig_Im_SMC}
\end{figure}
The results are essentially equivalent to the SIS results in \S \ref{Subs_SIS}.
Again we observe that the variance of the SMC estimate converges as $M \rightarrow \infty$ with the rate ${O}(1/M)$.


\subsubsection{Continuing to learn: data sets from further experiments}
\begin{figure}[h]
\centering
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=\linewidth]{smc_more_data.png}
  \end{minipage}
  \caption{Plots of the posterior density based on the 10 measurements given in Table \ref{Table_measurements} as well as a plot based on 40 further measurements.
  The posterior $\mu_{50}$ is more informed than the posterior $\mu_{10}$. Hence, the larger data set led to a reduction of the uncertainty in the parameter. }
  \label{Fig_10vs50}
\end{figure}
The data set presented in Table \ref{Table_measurements} is only one out of several data sets that were collected in independent experiments in the same experimental set-up.
The presented filtering problem is rather artificial, as a posterior update after the collection of every measurement (so once in each couple seconds) is not very realistic.
A more reasonable filtering problem is that of updating the posterior measure after each of the experiments has been fully performed. 
The posterior measure at time $t$ would then reflect the knowledge gained from $t$ independently performed experiments.

In Fig. \ref{Fig_10vs50} we compare the posterior density from \S \ref{Subsubsec_SMC} with a posterior density after six experiments with a total of 50 measurements.
The posterior measure after six experiments is more concentrated than the measure after one experiment.
This reflects less uncertainty in the parameter $g$ after seeing data from different experiments, which is consistent with our intuition about learning.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/4_outlook.tex <==
\section{Discussion}\label{sec:discussion}

\begin{itemize}
\item
Path degeneracy, too many updates decrease estimation quality; this is the fault of the particle filters, updating in general is a good idea 
\end{itemize}

In this section we describe two filtering problems, the pendulum and the tumor filtering problem. 
Both these problems are associated with real-world  experiments.
Throughout this tutorial we use the simple pendulum filtering problem to illustrate the filtering of model parameters.
The tumor filtering problem is discussed briefly to highlight a more involved application of filtering.


\begin{example}[Tumor]
The tumor inverse and filtering problem has been discussed extensively in the literature, see e.g. \cite{Collis2017, Kahle2018, Lima2017} and the references therein.
In this problem we model a tumor in a patient with a system of (partial) differential equations, for example, the Cahn-Hilliard or reaction-diffusion equations, or, alternatively, an atomistic model.
The goal is to predict the future growth of the tumor.
Moreover, we wish to test, compare and select suitable therapeutical treatments.
To do this we need to estimate model parameters, e.g. the tumor proliferation and consumption rate, and chemotaxis parameters.
These model parameters are patient-specific and can be calibrated and updated using patient data.
The data is given by tumor images obtained e.g. with \emph{magnetic resonance imaging} (MRI) or with \emph{positron emission tomography} (PET).
The images are captured at different timepoints and monitor the progression of the tumor growth.
Note that the data spaces are in general infinite-dimensional in this setting.
%The images can be used to calibrate and update the tumor model parameters.
%After each image is taken, the information from the image shall be learned and thus included in the model.
\end{example}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

==> sections/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
\bibliographystyle{spmpsci}
\bibliography{library}
%


